Personalized Subgraph Federated Learning

Subgraphs of a larger global graph may be distributed across multiple devices, and only locally accessible due to privacy restrictions, although there may be links between subgraphs. Recently proposed subgraph Federated Learning (FL) methods deal with those missing links across local subgraphs while distributively training Graph Neural Networks (GNNs) on them. However, they have overlooked the inevitable heterogeneity between subgraphs comprising different communities of a global graph, consequently collapsing the incompatible knowledge from local GNN models. To this end, we introduce a new subgraph FL problem, personalized subgraph FL, which focuses on the joint improvement of the interrelated local GNNs rather than learning a single global model, and propose a novel framework, FEDerated Personalized sUBgraph learning (FED-PUB), to tackle it. Since the server cannot access the subgraph in each client, FED-PUB utilizes functional embeddings of the local GNNs using random graphs as inputs to compute similarities between them, and use the similarities to perform weighted averaging for server-side aggregation. Further, it learns a personalized sparse mask at each client to select and update only the subgraph-relevant subset of the aggregated parameters. We validate our FED-PUB for its subgraph FL performance on six datasets, considering both non-overlapping and overlapping subgraphs, on which it significantly outperforms relevant baselines. Our code is available at https://github.com/JinheonBaek/FED-PUB.

==> algos/algo.tex <==
\begin{figure*}[h!]
    \begin{minipage}[t]{.495\linewidth}
        \begin{algorithm}[H]
        \small
    	\caption{\textbf{FED-PUB} Client Algorithm}
    	    \begin{algorithmic}[1]
    	        \label{algo:fedpub_client}
                \STATE  $R$: number of rounds, $E$: number of epochs, $K$: number of clients, $\mathcal{D}_k$: local data for client $k$. $\S(\cdot)$: similarity matching function, $\tau$: scaling factor for similarity matching, $\mu$: weight masking parameters. \\
                \vspace{0.095in}
                \STATE   \textbf{Function} RunClient($\bar{\theta}_{k}$)
                    \STATE $\theta_{k} \leftarrow \bar{\theta}_k \otimes \mu_k $ 
                    \FOR{each local epoch $e$ from $1$ to $E$}
                        \FOR{minibatch $\mathcal{B} \in \mathcal{D}_{k}$}
                            \STATE $\theta_k \leftarrow \theta_k-\eta\nabla\mathcal{L}(\mathcal{B}; \theta_k, \mu_k)$
                        \ENDFOR
                    \ENDFOR
                    \STATE \textbf{return} $\theta_k$
                    \vspace{0.01in}
                    
        	\end{algorithmic}
    	\end{algorithm}
    \end{minipage}
    \begin{minipage}[t]{.495\linewidth}
        \begin{algorithm}[H]
            \small
            \caption{\textbf{FED-PUB} Server Algorithm}
        	\begin{algorithmic}[1]
        	    \label{algo:fedpub_server}
        	   
                \STATE   \textbf{Function} RunServer()
                    \STATE initialize $\bar{\theta}^{(0)} $
                    \FOR{each round $r=1,2,\dots, R$}
                        \FOR{$f^{(r)}_k \forall k~\textbf{\mbox{in parallel}}$}
                            \IF{$r = 1$} 
                                \STATE $\theta_k^{(r+1)} \leftarrow \text{RunClient} (\bar{\theta}^{(r)})$
                            \ELSE
                                
                                \STATE $\bar{\theta}_{k}^{(r)} \leftarrow \sum_{i=0}^K \frac{\text{exp}({\tau \cdot S(i,k)})}{\sum_{i=0}^K \text{exp}(\tau \cdot S(i,k))}  \theta_i$
                                \STATE $\theta_k^{(r+1)} \leftarrow \text{RunClient} (\bar{\theta}_{k}^{(r)})$
                            \ENDIF 
                    	\ENDFOR
                    \ENDFOR 
                
        	\end{algorithmic}
    	\end{algorithm}
    \end{minipage}
    
\end{figure*}

==> figures/fig_analysis_lambda.tex <==
\begin{figure}[t]
    \small
    \centering
    \begin{minipage}{0.23\textwidth}
        % \hspace{-0.1in}
        \includegraphics[width=\textwidth]{figures/images/analisys_sparsity_cora.pdf} 
    \end{minipage}
    \begin{minipage}{0.25\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c c c c }
                \toprule 
        	    \midrule
        	    \centering
        	    \textbf{$\lambda_1$} & $\lambda_2$ & Sparsity [$\%$] & Accuracy [$\%$] \\
        	    \midrule
        	        1e-3 & 1e-3 & 41.98 $\pm$ 4.93 & 72.37	$\pm$ 0.18\\
         	    \midrule
                    1e-2 & 1e-3 & 53.33 $\pm$ 2.46 & 71.68	$\pm$ 0.35\\
                    1e-1 & 1e-3 & 69.31 $\pm$ 1.81 & 72.36	$\pm$ 1.65\\
                    3e-1 & 1e-3 & 80.70 $\pm$ 2.03 & \textbf{72.94	$\pm$ 0.85}\\
                    4e-1 & 1e-3 & 84.65 $\pm$ 0.84 & 70.52	$\pm$ 0.66\\
                    5e-1 & 1e-3 & \textbf{88.54 $\pm$ 0.77} & 68.65	$\pm$ 2.78\\
        	    \midrule
        	    \bottomrule 
            \end{tabular}
            \label{tbl:analysis_factorization_3}
        }
    \end{minipage}
    \begin{minipage}{0.25\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c c c c }
                \toprule 
        	    \midrule
        	    \centering
        	    $\lambda_1$ & \textbf{$\lambda_2$} & Sparsity [$\%$] & Accuracy [$\%$] \\
        	    \midrule
        	        1e-3 & 1e-3 & 41.98 $\pm$ 4.93 & 72.37	$\pm$ 0.18\\
         	    \midrule
                    1e-3 & 1e-2 & 39.79 $\pm$ 3.86 & 71.11	$\pm$ 0.79\\
                    1e-3 & 1e-1 & 39.45 $\pm$ 2.19 & 72.50	$\pm$ 0.68\\
                    1e-3 & 1 & 40.71 $\pm$ 3.28 & 72.44	$\pm$ 0.85\\
                    1e-3 & 20 & 42.39 $\pm$ 2.84 & \textbf{73.37	$\pm$ 1.02}\\
                    1e-3 & 100 & \textbf{43.00 $\pm$ 4.47} & 72.85	$\pm$ 0.56\\
                    
        	    \midrule
        	    \bottomrule 
            \end{tabular}
        \label{tbl:analysis_factorization_3}
        }
    \end{minipage}
    \begin{minipage}{0.25\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c c c c }
                \toprule 
        	    \midrule
        	    \centering
        	    \textbf{$\lambda_1$} & \textbf{$\lambda_2$} & Sparsity [$\%$] & Accuracy [$\%$] \\
        	    \midrule
        	        1e-3 & 1e-3 & 41.98 $\pm$ 4.93 & 72.37	$\pm$ 0.18\\
         	    \midrule
                    1e-2 & 1e-2 & 56.60 $\pm$ 1.58 & 72.33	$\pm$ 0.94\\
                    1e-1 & 1e-1 & 67.48 $\pm$ 2.33 & 73.10	$\pm$ 1.68\\
                    3e-1 & 1 & 81.74 $\pm$ 3.08 & 70.44	$\pm$ 1.81\\
                    3e-1 & 20 & \textbf{82.95 $\pm$ 0.64} & 72.16	$\pm$ 0.32\\
                    3e-1 & 30 & 81.80 $\pm$ 0.63 & \textbf{73.18 $\pm$ 0.61}\\
                    
        	    \midrule
        	    \bottomrule 
            \end{tabular}
        \label{tbl:analysis_factorization_3}
        }
    \end{minipage}
    \begin{tabular}{c c c c }
        (a) Model Sparsity 
        & \hspace{0.25in} (b) Effect of $\lambda_1$ 
        & \hspace{0.3in} (c) Effect of  $\lambda_2$ 
        & \hspace{0.15in} (d) Varying both $\lambda_1$ \& $\lambda_2$
    \end{tabular}
    \vspace{-0.1in}
    \caption{\textbf{Analysis on hyper-parameter $\lambda_1$ and $\lambda_2$} (a) Model sparsity curves controlled by $\lambda_1$ during training. Model sparsity and corresponding performance while varying (b) $\lambda_1$ only, (c) $\lambda_2$ only, and (d) both $\lambda_1$ and $\lambda_2$.}
    \label{fig:anlysis_lambda}
\end{figure}
